Asymptotic flatness in higher dimensions

We show that $(n+1)$-dimensional Myers-Perry metrics, $n\geq4$, have a conformal completion at spacelike infinity of $C^{n-3,1}$ differentiability class, and that the result is optimal in even spacetime dimensions. The associated asymptotic symmetries are presented.

==> MyersPerry.tex <==

\subsection{Odd spacetime dimensions}
 \label{ss31X21.1}

{\bluec
\ptcr{blue stuff version from Kubiznak \cite{FrolovKubiznak}, possibly useful, but to be ignored at this stage}

The Myers--Perry (MP) metrics   have slightly different form for the odd and even
number of spacetime dimensions $D$. We can write them compactly as
\begin{eqnarray}\label{MP}
ds^2&=&-dt^2+\frac{Udr^2}{V-2M}+\frac{2M}{U} (\,dt+
\sum_{i=1}^{n}a_i\mu_i^2d\phi_i)^{2} \non\\
&+&
\sum_{i=1}^{n}(r^2+a_i^2)(\mu_i^2d\phi_i^2
+d\mu_i^2)+\varepsilon r^2
d\mu^2_{n+\varepsilon}\, ,
\end{eqnarray}
where
\be
V=r^{\varepsilon-2}\prod_{i=1}^{n}(r^2+a_i^2)\hhh
U=V(1-\sum_{i=1}^n\frac{a_i^2 \mu_i^2}{r^2+a_i^2})\, .
\ee
Here $n=[(D-1)/2]$, where $[A]$ means the integer part of $A$. We
define $\varepsilon$ to be $1$ for $D$ even and $0$ for odd.   The
coordinates $\mu_i$ are not independent. They obey the following
constraint
%
\begin{equation}\label{constraint}
\sum_{i=1}^n\mu_{\!i}^2+\varepsilon \mu^2_{n+\varepsilon}=1.
\end{equation}
%
}


In Kerr-Schild-type coordinates the Myers-Perry metrics take the form~\cite{myersperry}
%
\begin{equation}\label{31X21.1}
  g_{\mu\nu} = \eta_{\mu\nu} + h k_\mu k_\nu
  \,,
\end{equation}
%
where $k_\mu$ is a null vector for the $(n+1)$-dimensional Minkowski metric $\eta$, and hence also for the full metric:
%
\begin{equation}\label{31X21.1}
  g^{\mu\nu} = \eta^{\mu\nu} - h k^\mu k^\nu
  \,,
 \quad
 \eta^{\mu\nu}k_\mu k_\nu=g^{\mu\nu}k_\mu k_\nu=0
  \,,
 \quad
 k^\nu = \eta^{\mu\nu}k_\mu =g^{\mu\nu}k_\mu
  \,.
\end{equation}
%

Let the space-dimension $n=2d\ge 4$ be even,
 \ptcr{what happens if $n=2$?}
 and choose coordinates
 \ptc{here I am using angles which are not the same as  the second part of the MP paper}
%
\begin{eqnarray}
 (x^\mu)  &\equiv& (x^0,x^i) = (t,x_1,y_1,\ldots,x_d,y_d)
    \nonumber
     \\
    &=&  \big(t, r_1 \cos(\varphi_1),  r_1 \sin (\varphi_1), \ldots,r_d \cos(\varphi_d),  r_d \sin (\varphi_d)
  \big)
\end{eqnarray}
%
in which the Minkowski metric takes the form
%
$$
\eta = -dt^2 + \sum_{i=1}^{d} (dx_i^2+dy_i^2)= -dt^2 + \sum_{i=1}^{d} (dr_i^2+r_i^2 d\varphi_i^2)
\,.
$$
%
In these coordinates the vector field $k$ and the function $h$ read
%
\begin{eqnarray}
  k_\alpha  dx^\alpha &=&
   dt + \sum_{i=1}^{d}  \frac{\rMP (x_i dx_i + y_i dy_i) +a_i (x_i dy_i - y_i dx_i) }{\rMP ^2+a_i^2}
\\ &=&
   dt + \sum_{i=1}^{d}  \frac{\rMP r_i dr_i + a_i r_i^2   d\varphi_i  }{\rMP ^2+a_i^2}
    \,,
\\
  h &=& \frac{\muMP  \rMP ^2}{\Pi F}
   \,,
\\
  F &=& 1 - \sum_{i=1}^{d}\frac{a_i^2(x_i^2+y_i^2)}{(\rMP ^2+a_i^2)^2}
  \,,
\\
  \Pi &=&  \prod_{i=1}^{d} (\rMP ^2+a_i^2)
  \,,
   \label{31X21.6}
\end{eqnarray}
%
with a set of constants $\muMPhalf ,\, a_i\in \R$.
Finally, the function $\rMP $ is defined implicitly by the condition that $k$ is null:
%\ptcheck{31X}
%
\begin{equation}\label{31X21.7}
  \sum_{i=1}^{d}\frac{ x_i^2+y_i^2 }{\rMP ^2+a_i^2} = 1
  \,.
\end{equation}
%
Letting
%
$$
 r^2 := \sum_{i=1}^{d} r_i^2
  \equiv \sum_{i=1}^{d} (  x_i^2+y_i^2)
 \,,
 \qquad
 \,,
$$
%
one finds the asymptotic expansions, for large $r$,
%
\begin{eqnarray}\label{31X21.8}
  \rMP^2
   & = &
    r^2  - \sum_{i=1}^{d} \frac{a_i^2r_i^2}{r^2} + O(r^{-2})
    =
    r^2\big(1 + O(r^{-2})
  \big)
    \,,
\\
 F & = & 1 + O(r^{-2})
    \,,
\\
 \Pi & = & r^{n}\big(1 + O(r^{-2})
  \big)
    \,,
\\
 h & = &  \frac{\muMP }{r^{  n-2 }}\big(1 + O(r^{-2})
  \big)
\\
  g &=&  \eta + \frac{\muMP }{r^{  n-2 }}\Big(
   dt^2
  +
   2dt \sum_{i=1}^{d}  \frac{ rr_i dr_i +a_i r_i^2 d\varphi_i  }{r^2}
  \nonumber
\\
 &&
  +
     \sum_{i,j=1 }^{d}  \frac{
     \big(
      rr_i dr_i +a_i r_i^2 d\varphi_i
      \big)
     \big(
      rr_j dr_j +a_j r_j^2 d\varphi_j
      \big)
      }{r^4 }
  \nonumber
\\
   &&
  + O(r^{-2}) dx^\mu    dx^\nu
  \Big)
  \,.
\end{eqnarray}
%
We see from the last equation that the metric is asymptotically flat at spatial infinity, with well defined energy, but the mixed time-space metric functions decay slower by one power of $r$ than usually expected. This can be remedied by a  fine-tuning of the coordinates, but will not be necessary for our purposes.

We can carry out a variant of the calculations of Section~\ref{s31X32.2}, as follows: We write the metric as  in \eqref{31X21.1} and perform a Kelvin transformation as in \eqref{30IX21.5}, with $\rstar$ there replaced by $r$,
%
\begin{equation}\label{30IX21.6435}
 t= \frac{\tau}{\rho^2 - \tau^2}
 \,,
 \qquad
 r = \frac{\rho }{\rho^2 - \tau^2}
\,,
\end{equation}
%
to obtain:
%
\begin{eqnarray}
  g &=& \eta +  h\,  k \otimes k
     \nonumber
\\
 &=&
   \underbrace{\frac{1}{(\rho^2-\tau^2)^2 }
    }_{=:\Omega^{-2}}
    \Big(
    \underbrace{
     - d\tau^2 + d\rho^2 + \rho^2 d\Omega^2_{n-1}
      }_{\eta}
     +  (\rho^2-\tau^2)^2
     h\,  k \otimes k
     \Big)
   \,.
   \phantom{xxxx}
\end{eqnarray}
%
To understand the properties of $\Omega^2 g$ at
%
\begin{equation}\label{1X21.12}
 \red{i_0}:=\{\rho=\tau=0\}
\end{equation}
%
we need to analyse the   function $h$ and the covector field
%
\begin{equation}\label{1X21.11}
     \tilde  k := (\rho^2-\tau^2) k
     \,.
\end{equation}
%
For this we return to  \eqref{31X21.7}, which after setting
%
$$
 r_i = r \, m_i
 \,,
 \qquad
 x= 1/r\,,
 \qquad\xMP:= 1/\rMP
% \,,
$$
%
(thus  $\sum_{i=1}^d m_i^2 =1$),   can be rewritten as
%
\begin{equation}\label{31X21.72}
   \xMP \underbrace{
    \sqrt{
     \sum_{i=1}^{d}\frac{ m_i^2 }{1+a_i^2\xMP^2 }
     }
    }_{=: f_1(\xMP^2,m_i)} = x
  \,.
\end{equation}
%
The function $0< f_1 \le 1$ is real analytic, with $f_1(0,m_i)=1$. One easily checks that $\xMP\mapsto \xMP f_1(\xMP^2)$ is strictly increasing  so that, for any given set $(m_i)$, by the (analytic) inverse function theorem there exists a real-analytic function $s\mapsto f_2(s,m_i)>0$ solving \eqref{31X21.72}
%
\begin{equation}\label{31X21.73}
   \xMP  =  x f_2(x^2,m_i)\,, \ \mbox{with} \ f_2(0,m_i)=1
  \,.
\end{equation}
%
In terms of $(\tau,\rho)$ coordinates this reads
%
\begin{equation}\label{31X21.73}
   \rMP = \frac{
    1}{
       \rho \big( 1 - \frac{\tau^2}{\rho^2}
     \big) f_2\big(\rho^2(1 - \frac{\tau^2}{\rho^2})^2,m_i\big)}=:
     \frac{ f_3(\tau^2,\rho^2,m_i)}{ \rho \big( 1 - \frac{\tau^2}{\rho^2}
     \big)}
      \,, \ \mbox{with} \ f_3(0,0,m_i)=1
  \,.
\end{equation}
%
As in the Schwarzchild case we are only interested in the region $|\tau/\rho|\le 1$, it is therefore convenient to extend the function $1-\tau^2/\rho^2$ beyond this region to a smooth function which is constant for $|\tau/\rho|\ge 2$. Then the function $f_3$ is a smooth function of its arguments on the set
%
$$\mcO:=\{\tau^2+\rho^2<\epsilon\}\times\{(m_i)\in S^{d}\}
\,,
$$
%
for some $\epsilon>0$.  It also follows that
%
\begin{equation}\label{1XI21.31}
  \mbox{the functions $r^{-2}$, $\rMP^{-2}$, $r/\rMP$ and $\rMP/r$ are smooth on $\mcO$, with $r/\rMP|_{i_0}=1$.}
\end{equation}




==> MyersPerry2.tex <==
One now checks that there exist functions $f_{\cdot}$, all smooth on $\mcO$, such that:
%
\begin{eqnarray}
 F & = & 1- \sum_{i=1}^{d}\frac{a_i^2r^2 m_i^2 }{(\rMP ^2+a_i^2)^2}
  = 1 - \rho^2 f_4
    \,,
\\
 \Pi^{-1} & = &  \prod_{i=1}^{d} (\rMP ^2+a_i^2)^{-1}
 = \rho ^{n}
  \big(1 - \frac{\tau^2}{\rho^2}\big)^n \big(1 + \rho^2f_5)
  \big)
    \,,
\\
 h & = & \frac{\muMP  \rMP ^2}{\Pi F}=
  \muMP \rho ^{n-2}
  \big(1 - \frac{\tau^2}{\rho^2}\big)^{n-2} \big(1 + \rho^2f_6 
  \big)
  \,,
\\
 \tilde k  &=&  \rho^2 \big(1-\frac{\tau^2}{\rho^2}\big)
 \big(
    dt +  \sum_{i=1}^{d}  \frac{ \rMP r_i dr_i +a_ir_i^2 d\varphi_i }{\rMP^2 + a_i^2}
    \big)
  \nonumber
\\
&=&  \rho^2 \big(1-\frac{\tau^2}{\rho^2}\big)
 \Big(
    dt +  \sum_{i=1}^{d} \big(
       m_i d(r m_i)(1+\rho^2 f_{7,i})
         +a_i m_i^2 (1+\rho^2 f_{8,i}) d\varphi_i
    \big)
    \Big)
  \nonumber
\\
&=&
\rho^2 \big(1-\frac{\tau^2}{\rho^2}\big)
 \Big(
    \underbrace{d(t + r)}_{(d\tau-d\rho)(\rho-\tau)^{-2}} +  \underbrace{ \sum_{i=1}^{d} \big(
       r m_i d  m_i}_{=0}
       +
       \underbrace{
        \rho^2 f_{7,i}  m_i d(r m_i) }
         _{
        \rho^3 f_{9,i}  m_i d m_i   /(\rho^2-\tau^2)   +
        \rho^2 f_{7,i}  m_i^2  d r  }
  \nonumber
\\
& &
         +a_i m_i^2 (1+\rho^2 f_{8,i}) d\varphi_i
         \big)
    \Big)
  \nonumber
\\
&=&
 \frac{1+\frac{\tau}{\rho}}{1-\frac{\tau}{\rho}}
 (d\tau-d\rho)
    + 
    \sum_{i=1}^{d} \Big(
        \rho^3  f_{9,i}  m_i d m_i 
  \nonumber
\\
& & 
    + \rho^2 \big(1-\frac{\tau^2}{\rho^2}\big)
 \big(
        \rho^2 f_{7,i}  m_i^2  d r
         +a_i m_i^2 (1+\rho^2 f_{8,i}) d\varphi_i
         \big)
    \Big) 
  \,.
\end{eqnarray}
%
Using
%
\begin{equation}\label{1X21.51}
  dr = 
    \rho^{-2}\big(1-\frac{\tau^2}{\rho^2}\big)^{-2} 
  \big( \frac{2\tau}{\rho } d\tau -  \big(1+\frac{\tau^2}{\rho^2}\big) d\rho
  \big)
  \,,
\end{equation}
%
we can rewrite $\tilde k$ as
%
\begin{eqnarray}
 \tilde k
&=&
 \frac{1+\frac{\tau}{\rho}}{1-\frac{\tau}{\rho}}
 (d\tau-d\rho)
   +   
   \sum_{i=1}^{d} \big(
        \rho^3 f_{9,i}  m_i d m_i
         +a_i \rho^2 m_i^2
         f_{10,i}
         %\big(1-\frac{\tau^2}{\rho^2}\big)
   % (1+\rho^2 f_{8,i})
   d\varphi_i
    \big)
    \Big) 
  \nonumber
\\
& & + 
       \frac{1}{1-\frac{\tau^2}{\rho^2}}
         \sum_{i=1}^{d}    f_{7,i}  m_i^2
        \big( 2 \rho \tau d \tau
        -   \big(\rho^2 + \tau^2) d\rho
        \big)
  \,.
\end{eqnarray}
%
It follows that $h\,\tilde k \otimes \tilde k$ takes the form 
%
\begin{eqnarray}
% \nonumber % Remove numbering (before each equation)
  h \, \tilde k \otimes \tilde k &=& \muMP  \rho^{n-2} \big(1-\frac{\tau^2}{\rho^2}\big)^{n-4} \psi_{\mu\nu} dy^\mu dy^\nu
  \,,
\end{eqnarray}
%
where $(y^\mu)\equiv (y^0,y^i):= (\tau, \rho m^i)$, and where the functions $\psi_{\mu\nu}$ satisfy, for all $\alpha\in \N^{n+1}$,
%
$$ \rho ^{\alpha_0+\ldots +\alpha_n} (\partial_{y^0}) ^{\alpha_0 }
 \cdots
(\partial_{y^n} )^{\alpha_n }
  \psi_{\mu\nu}=O(1)
\,.
$$
% 
Keeping in mind that  in this section $n\ge 4$, this leads again to a conformally extended metric of differentiability class $C^{n-3,1}$. 

==> PTCTheoremsForOxford2.tex <==

% Custom theorem styles (WARNING: require \usepackage{amsthm})

\newtheoremstyle{normal} % name
  {5pt} % Space above
  {5pt} % Space below
  {\rm} % Body font
  {} % Indent amount
  {\sc} % Theorem head font
  {} % Punctuation after theorem head
  {0.5em} % Space after theorem head
  {} % Theorem head spec

\newtheoremstyle{italics} % name
  {5pt} % Space above
  {5pt} % Space below
  {\it} % Body font
  {} % Indent amount
  {\sc} % Theorem head font
  {} % Punctuation after theorem head
  {0.5em} % Space after theorem head
  {} % Theorem head spec

\newtheoremstyle{indentnormal} % name
  {5pt} % Space above
  {5pt} % Space below
  {\addtolength{\leftskip}{1.5 em}\rm} % Body font
  {} % Indent amount
  {\sc} % Theorem head font
  {} % Punctuation after theorem head
  {0.5em} % Space after theorem head
  {} % Theorem head spec

\newtheoremstyle{indentitalics} % name
  {5pt} % Space above
  {5pt} % Space below
  {\addtolength{\leftskip}{1.5 em}\it} % Body font
  {} % Indent amount
  {\sc} % Theorem head font
  {} % Punctuation after theorem head
  {0.5em} % Space after theorem head
  {} % Theorem head spec

\newtheoremstyle{indentnormalsmall} % name
  {5pt} % Space above
  {5pt} % Space below
  {\addtolength{\leftskip}{1.5 em}\rm\small} % Body font
  {} % Indent amount
  {\sc} % Theorem head font
  {} % Punctuation after theorem head
  {0.5em} % Space after theorem head
  {} % Theorem head spec

\newtheoremstyle{indentnormalsmallvoid} % name
  {5pt} % Space above
  {5pt} % Space below
  {\addtolength{\leftskip}{1.5 em}\rm\small} % Body font
  {} % Indent amount
  {\sc} % Theorem head font
  {} % Punctuation after theorem head
  {0em} % Space after theorem head
  {} % Theorem head spec



% To redefine theorems (taken from https://tex.stackexchange.com/questions/103013/)
\makeatletter
\def\renewtheorem#1{%
  \expandafter\let\csname#1\endcsname\relax
  \expandafter\let\csname c@#1\endcsname\relax
  \gdef\renewtheorem@envname{#1}
  \renewtheorem@secpar
}
\def\renewtheorem@secpar{\@ifnextchar[{\renewtheorem@numberedlike}{\renewtheorem@nonumberedlike}}
\def\renewtheorem@numberedlike[#1]#2{\newtheorem{\renewtheorem@envname}[#1]{#2}}
\def\renewtheorem@nonumberedlike#1{
\def\renewtheorem@caption{#1}
\edef\renewtheorem@nowithin{\noexpand\newtheorem{\renewtheorem@envname}{\renewtheorem@caption}}
\renewtheorem@thirdpar
}
\def\renewtheorem@thirdpar{\@ifnextchar[{\renewtheorem@within}{\renewtheorem@nowithin}}
\def\renewtheorem@within[#1]{\renewtheorem@nowithin[#1]}
\makeatother

% WARNING: there was a problem with theorem, lemma, proposition,
% example, and remark (I have to use \renewtheorem on them) probably
% this is due to the modification in the OUP style file)


%\renewtheorem{theorem}{Theorem}[section]%{{\sc \color{red}{Theorem}\rm}}[section]%{\sc Theorem\rm}%
% \renewtheorem{definition}[theorem]{Definition}
%\renewtheorem{lemma}[theorem]{\sc Lemma\rm}
%\renewtheorem{example}[theorem]{\sc Example\rm}
% % 'Examples' use same counter as 'Example'
% \renewtheorem{examples}[theorem]{Examples}
% \renewtheorem{corollary}[theorem]{Corollary}
%\renewtheorem{remark}[theorem]{\sc Remark\rm}
%\renewtheorem{proposition}[theorem]{\sc Proposition\rm}


% MM: do we need these?

\newtheorem{Theorem} {\sc {Theorem}\rm}[section]
%\newtheorem{theorem} [Theorem] {\sc  Theorem\rm}
\newtheorem{theo} [Theorem] {\sc  Theorem\rm}
\newtheorem{cor} [Theorem] {\sc  Corollary\rm}
\newtheorem{Corollary} [Theorem] {\sc  Corollary\rm}
\newtheorem{Lemma} [Theorem] {\sc  Lemma\rm}
%\newtheorem{Proposition} [Theorem] {\sc  Proposition\rm}
\newtheorem{prop} [Theorem] {\sc  Proposition\rm}
\newtheorem{pro} [Theorem] {\sc  Proposition\rm}
\newtheorem{Conjecture}[Theorem]{\sc  Conjecture\rm}
\newtheorem{conjecture}[Theorem]{\sc  Conjecture\rm}
\newtheorem{Definition}[Theorem]{\sc  Definition\rm}
%\newtheorem{definition}[Theorem]{\sc  Definition\rm}


\newtheorem{lemm}[Theorem]{\sc Lemma\rm}
\newtheorem{coro}[Theorem]{\sc Corollary\rm}

% \newtheorem{lemma} [Theorem] {\sc  Lemma\rm}

\newtheorem{lem} [Theorem] {\sc  Lemma\rm}
% \newtheorem{proposition} [Theorem] {\sc  Proposition\rm}
\newtheorem{Def}[Theorem]{\sc  Definition\rm}

\newtheorem{thm}[Theorem]{\sc  Theorem\rm}

\newtheorem{Proposition} [Theorem] {\sc  Proposition\rm}

\newtheorem{ptcproposition}  [Theorem] {\sc  Proposition\rm}
\newtheorem{aptctheorem} {\sc  Theorem\rm} [section]
\newtheorem{aptcproposition} [aptctheorem]  {\sc  Proposition\rm}
\newtheorem{aptccorollary} [aptctheorem] {\sc  Corollary\rm}
\renewcommand{\theaptctheorem}{A.\arabic{aptctheorem}}



\newtheorem{ptcTheorem} {\sc  Theorem\rm} [section]
\newtheorem{ptctheorem} [Theorem] {\sc  Theorem\rm}
\newtheorem{ptctheo} [Theorem] {\sc  Theorem\rm}
\newtheorem{ptccor} [Theorem] {\sc  Corollary\rm}
\newtheorem{ptcCorollary} [Theorem] {\sc  Corollary\rm}
\newtheorem{ptcLemma} [Theorem] {\sc  Lemma\rm}
\newtheorem{ptcProposition} [Theorem] {\sc  Proposition\rm}
\newtheorem{ptcprop} [Theorem] {\sc  Proposition\rm}
\newtheorem{ptcpro} [Theorem] {\sc  Proposition\rm}
\newtheorem{ptcConjecture}[Theorem]{\sc  Conjecture\rm}
\newtheorem{ptcconjecture}[Theorem]{\sc  Conjecture\rm}
\newtheorem{ptcDefinition}[Theorem]{\sc  Definition\rm}
\newtheorem{ptcdefinition}[Theorem]{\sc  Definition\rm}
% \theoremstyle{Remark}

%
% odtad wszystko jest prosta trzcionka
%
%

% \theorembodyfont{\upshape}
\theoremstyle{normal}
\newtheorem{adc}[Theorem]{\sc Asymptotic decay conditions\rm}
\newtheorem{Remark}[Theorem]{\sc Remark\rm}
% \newtheorem{remark}[Theorem]{\sc Remark\rm}
\newtheorem{Remarks}[Theorem]{\sc Remarks\rm}
\newtheorem{remk}[Theorem]{\sc Remark\rm}
\newtheorem{remks}[Theorem]{\sc Remarks\rm}
% \newtheorem{example}[Theorem]{\sc Example\rm}
\newtheorem{Example} [Theorem] {\sc Example\rm}
\newtheorem{Problem}[Theorem]{\sc Problem\rm}
\newtheorem{Exercise}[Theorem]{\sc Exercise\rm}


%
% odtad wszystko jest mniejsza trzcionka, ale ciagle prosta
%
\theoremstyle{indentnormalsmall}
% \theoremsymbol{\ensuremath{\diamondsuit}}
\newcommand{\fcoco}{\small}
% \theorembodyfont{\fcoco}\theoremseparator{}\theoremindent0.5cm
\newtheorem{cocoEx}[Theorem]{\sc Exercise\rm}
\newtheorem{cocoPr}[Theorem]{\sc Problem\rm}
\newtheorem{cocoProposition}[Theorem]{\sc Proposition\rm}
\newtheorem{cocoProp}[Theorem]{\sc Proposition\rm}
\newtheorem{cocoprop}[Theorem]{\sc Proposition\rm}
\newtheorem{cocoRm}[Theorem]{\sc Remark\rm}
\newtheorem{cocoExa}[Theorem]{\sc Example\rm}
\newtheorem{cocoTh}[Theorem]{\sc  Theorem\rm}
\newtheorem{cocoRem}[Theorem]{\sc  Remark\rm}
\newtheorem{cocoRemark}[Theorem]{\sc  Remark\rm}
\newtheorem{cocorem}[Theorem]{\sc  Remark\rm}
\newtheorem{cocoCorollary}[Theorem]{\sc Corollary\rm}
% \theoremstyle{nonumberplain}\theorembodyfont{\fcoco}
% \theoremseparator{}\theoremindent0.5cm
%\newtheorem{coco}{}
\newtheorem*{coco}{\sc {\color{blue} Incidentally:}%
%(coco environement, to be thought over):}
\rm}

\newtheorem*{SmallerIndented}{\hspace{-.5em}}%{%
\newtheorem*{coc}{\hspace{-.5em}}%{%

%

% \theoremstyle{definition}
\newtheorem{defi}[Theorem]{\sc Definition\rm}
\newtheorem{notn}[Theorem]{\sc Notation\rm}
\newtheorem{conj}[Theorem]{\sc Conjecture\rm}

\theoremstyle{indentnormalsmallvoid}
\newtheorem*{cocnoind}{}%{%
%(coco environement, to be thought over):}
%\rm}


==> deflection.tex <==
\subsection{Deflection angle}

The \emph{total deflection angle}, say $\varphi_\gamma$, along $\gamma$ equals
%
\begin{equation}\label{2X21.5}
  \varphi_\gamma := \int_{-\infty}^{\infty} \frac{d\varphi}{ds} ds
   = 2 \int_{b}^{\infty} \frac{d\varphi}{dr} dr
   \,.
\end{equation}
%
Equation~\eq{2X21.3}
 implies, changing $\varphi$ to $-\varphi$ if necessary,
%
\begin{equation}\label{2X21.3}
   \frac{d\varphi}{dr} = \frac{ J}{r \sqrt{r^2 - J^2  + \frac{2mJ^2}{r^{n-2}}}}
   \,.
\end{equation}
%
Thus
 \ptcr{watch out, a non-trivial limit to take, and maybe infinity so one needs to first simplify things; if $m=0$ the last line is $\pi/(2J)$}
%
\begin{eqnarray}
  \varphi_\gamma
   &   = &
     2J \int_{b}^{\infty}
      \frac{dr}{r \sqrt{r^2 - J^2  + \frac{2mJ^2}{r^{n-2}}}}
      \nonumber
\\
   &   = &
     2J \int_{b}^{\infty}
     \left(
      \frac{1}{r \sqrt{r^2 - J^2  + \frac{2mJ^2}{r^{n-2}}}}
      -
      \frac{1}{r \sqrt{r^2 - J^2  + \frac{2mJ^2}{b^{n-2}}}}
      +
      \frac{1}{r \sqrt{r^2 - J^2  + \frac{2mJ^2}{b^{n-2}}}}
      \right)
      dr
      \nonumber
\\
   &   = &
     2J \int_{b}^{\infty}
     \left(
      \frac{1}{r \sqrt{r^2 - J^2  + \frac{2mJ^2}{r^{n-2}}}}
      -
      \frac{1}{r \sqrt{r^2 - J^2  + \frac{2mJ^2}{b^{n-2}}}}
      \right)
      dr
 \nonumber
\\
 &&
      +\underbrace{\frac{2 r b^{n/2} \sqrt{J^2 \left(2 m b^{-n}-\frac{1}{r^2}\right)+1} \cot ^{-1}\left(\frac{J b^{n/2}}{\sqrt{b^n
   \left(r^2-J^2\right)+2 J^2 m r^2}}\right)}{\sqrt{b^n \left(r^2-J^2\right)+2 J^2 m r^2}}
   \Bigg|^\infty_b
   }_{=\pi}
   \,.
   \label{2X21.5}
\end{eqnarray}
%


